New determination of the production cross section for secondary positrons and electrons in the Galaxy

The cosmic-ray fluxes of electrons and positrons ($e^{\pm}$) are measured with high precision by the space-borne particle spectrometer AMS-02. To infer a precise interpretation of the production processes for $e^{\pm}$ in our Galaxy, it is necessary to have an accurate description of the secondary component, produced by the interaction of cosmic-ray proton and helium with the interstellar medium atoms. We determine new analytical functions of the Lorentz invariant cross section for the production of $\pi^\pm$ and $K^\pm$ by fitting data from collider experiments. We also evaluate the invariant cross sections for several other channels, involving for example hyperon decays, contributing at the few \% level on the total cross section. For all these particles, the relevant 2 and 3 body decay channels are implemented, with the polarized $\mu^\pm$ decay computed with next-to-leading order corrections. The cross section for scattering of nuclei heavier than protons is modeled by fitting data on $p+C$ collisions. The total differential cross section $d\sigma/dT_{e^\pm}(p+p\rightarrow e^\pm+X)$ is predicted from 10 MeV up to 10 TeV of $e^\pm$ energy with an uncertainty of about 5-7\% in the energies relevant for AMS-02 positron flux, thus dramatically reducing the precision of the theoretical model with respect to the state of the art. Finally, we provide a prediction for the secondary Galactic $e^\pm$ source spectrum with an uncertainty of the same level. As a service for the scientific community, we provide numerical tables and a script to calculate energy-differential cross sections.

==> aps-length <==
#!/usr/bin/env python

"""
Count length of an APS manuscript formatted in LaTeX, following
guidelines described at http://journals.aps.org/authors/length-guide

Copyright (c) James Kermode <james.kermode@gmail.com> 2014

This program is free software; you can redistribute it and/or modify
it under the terms of the GNU General Public License as published by
the Free Software Foundation; either version 2 of the License, or
(at your option) any later version.

This program is distributed in the hope that it will be useful,
but WITHOUT ANY WARRANTY; without even the implied warranty of
MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
GNU General Public License for more details.

You should have received a copy of the GNU General Public License along
with this program; if not, write to the Free Software Foundation, Inc.,
51 Franklin Street, Fifth Floor, Boston, MA 02110-1301 USA.
"""

import glob
import optparse
import os
import sys
import subprocess

word_limit = {'PRL':    3750,
              'PRA-RC': 4500,
              'PRB-RC': 3500,
              'PRC-RC': 4500,
              'PRD-RC': 4500,
              'PRE-RC': 4500,
              'PRApplied': 3500,
              'PRST-PER':  3500}
# word limits from: https://journals.aps.org/authors/length-guide
# updated 2017-10-03

wordcount_tex_contents = r"""\ProvidesFile{wordcount.tex}[2000/09/27 v1.5 Michael Downes]
% Copyright 2000 Michael John Downes
% This file has no restrictions on its use, distribution, or sale.
%
% If you run LaTeX on wordcount.tex it will prompt you for the name of a
% document to be counted. For most people, however, it will be more
% convenient to run the shell script wordcount.sh, giving the document
% name as the first argument. The comments in wordcount.sh
% give further information about the usage and limitations of this tool.

% The fundamental idea is to mark each character and interword space
% with a unique tag that will show up in TeX "showbox" output. Then
% arrange to make the output routine trigger a TeX overfull vbox message
% for the page box so that everything gets reported in the TeX log.
% Then run grep -c (or an equivalent text search utility, e.g., perl) on
% the log file to count the occurrences.
%
% In showbox output, a character is typically represented by a line of
% the form
%
%   ...\T1/cmr/m/n/10 e
%
% where "\T1/cmr/m/n/10" is the font name. We arrange things so that all
% characters are typeset in a font named "\3.08632". Furthermore, for
% interword spaces, which are normally represented in the output as
% something like
%
%   ...\glue 3.33333 plus 1.66666 minus 1.11111
%
% we use \spaceskip to ensure that it always appears as
%
%   ...\glue(\spaceskip) 3.08633 plus 9.0
%
% Then to count characters (including word spaces) we can
% grep for lines matching "3.0863", while to count words we
% count the number of lines in the log that match "3.08633" but not
% "3.08632".
%
% For an accurate count in multi-line paragraphs we also need
% to set rightskip to the flag value, since interword spaces are
% discarded at line breaks; and on the presumption that hyphenated
% compounds like "steady-state" should be counted as two words, we set
% \exhyphenpenalty to a value that ensures a line break at *every*
% explicit hyphen---then we will get a rightskip glue node between the
% two parts. (How about em-dashes? you may ask. Answer: it works all
% right, try it and see.)

\ifx\relax\?\def\wcQUIET{TT}\else\def\wcQUIET{TF}\fi

% We want accented letters to be represented by a single font char, to
% the extent possible:
\RequirePackage[T1]{fontenc}
\makeatletter
\thickmuskip=5.55555mu plus5.55555mu minus 2.22222mu
\let\@@thickmuskip\thickmuskip \newmuskip\thickmuskip
\let\@@spaceskip\spaceskip \xspaceskip=0pt
\newskip\@charfontname
% Ensure that these cannot be overridden.
\let\spaceskip\@charfontname \let\xspaceskip\spaceskip
\def\FreezeSpaces{%
  \setbox\z@\hbox{\mathsurround=\z@ $\mkern\@@thickmuskip$}%
  \@@spaceskip=\wd\z@ plus 9pt\relax
  % Setting rightskip to a slightly different value means that
  % end-of-line spaces can be distinguished if desired. (By default,
  % they are not.) Using fil units means there won't be any hyphenation
  % except for explicit hyphens.
  \dimen@\@@spaceskip \advance\dimen@ 1sp\relax
  \rightskip\z@ plus\strip@pt\dimen@ fil\relax
  % Prevent any further changes to \rightskip.
  \let\rightskip\spaceskip
  \@charfontname=\wd\z@ \advance\@charfontname -1sp\relax
  % Cancel all non-1000 sfcodes, which might otherwise affect the value
  % of inter-sentence spaces and keep them from being counted as
  % interword spaces.
  \def\do{\sfcode\fam\@m \advance\fam\@ne
    \ifnum\fam>\@cclv\expandafter\@gobble\fi \do
  }%
  \fam\z@ \do
  \let\frenchspacing\relax \let\nonfrenchspacing\relax
}
\def\DashPatch{%
  \exhyphenpenalty=-\@M \let\exhyphenpenalty\count@
  \hyphenpenalty\@M \let\hyphenpenalty\count@
  % LaTeX bug? Default definitions for these don't have \exhyphenpenalty
  % built in. Change them to just print a hyphen so that the penalties
  % will work.
  \def\textemdash{-}\def\textendash{-}%
}
% Here we set the font to ptmr8t (a T1 encoded font for which most
% people are likely to have a tfm file) and then make it difficult for
% the font to be changed ever again. We use two names for the font,
% \ptmr and \3.08632, the former being easier to use when resetting math
% fonts. The name that is defined last when TeX processes a document is
% the one that will be used in the log file.
\def\FreezeFont{%
  \expandafter\font
    \csname\strip@pt\@charfontname\endcsname
    =ptmr8t \relax
  \ptmr
  \check@mathfonts \let\check@mathfonts\relax
  \def\do{%
    \textfont\fam=\ptmr\scriptfont\fam=\ptmr\scriptscriptfont\fam=\ptmr
    \advance\fam\@ne \ifnum\fam<\sixt@@n \else\expandafter\@gobble\fi
    \do
  }%
  \fam=0 \do
}
\font\ptmr=ptmr8t \relax
\fontdimen22\ptmr=1sp % to permit use as math font 2
\let\selectfont\relax
\let\fontshape\@gobble \let\fontseries\@gobble \let\fontfamily\@gobble
\let\fontencoding\@gobble \let\fontsize\@gobbletwo
\let\linespread\@gobble
\let\try@load@fontshape\relax
\@namedef{U/msa/m/n}{}% disable special test in AMS documentclasses
\def\define@newfont{\expandafter\let\font@name=\ptmr}
\let\@@hfuzz\hfuzz \let\@@vfuzz\vfuzz
\newdimen\hfuzz \let\vfuzz\hfuzz
\def\QuietBoxes{%
  \@@hfuzz\maxdimen \@@vfuzz\maxdimen
}
\AtBeginDocument{\FreezeSpaces \FreezeFont \DashPatch \QuietBoxes}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Halign patches
\def\ialign{\everycr{}\tabskip\@@spaceskip\halign} % initialized \halign
\def\extracolsep#1{\tabskip\@@spaceskip}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\nofiles \let\makeindex\@empty % work-around for a natbib problem
% Seize control of the output routine to avoid extra clutter of dvi
% files. Handling \AtBeginDVI would take some extra work--for now I
% won't bother.
\def\showpagebox{%
  \showboxbreadth\maxdimen\showboxdepth99
  % This is a devious way of getting the box contents into the log file
  % without actually using \showbox (which typically results in a
  % nonzero exit code from the TeX run).
  \@@vfuzz\z@
  \setbox\z@\vbox to\z@{\box\@outputbox}%
  \setbox\z@\box\voidb@x
  \global \@colht \textheight
  \stepcounter{page}%
  \let\firstmark\botmark
}
\AtBeginDocument{\def\@outputpage{\showpagebox}}
\if\wcQUIET\else
\begingroup \def\msg^^J#1]^^J{\endgroup\message{#1]^^J^^J}}
\endlinechar=`\^^J \catcode`\ =12 \msg

The 'wordcount' utility provides a way of estimating the number of
words in a LaTeX document.

[Warning: The counting method uses a large log file as an intermediate
step. If your disk space is extremely low the counting process
may end prematurely for lack of space.]

\fi

% \typein has extraneous blank lines and slightly idiosyncratic prompt.
\begingroup \endlinechar=-1
\message{File name [press RETURN to cancel]: }
\def\do{%
  \let\do\@makeother \dospecials
  \global\read-1 to\wcFileName
  \endgroup
}
\do

\ifx\@empty\wcFileName
  \typeout{No file name given; quitting.}\expandafter\@@end\fi

\expandafter\filename@parse\expandafter{\wcFileName}
\edef\jobname{\filename@base}

\if\wcQUIET
  \message{\wcFileName}
\else
\typeout{^^JTo get a count of characters, run^^J^^J \space
%
  grep -c '3[.]0863[23]' wordcount.log^^J^^J%
%
or equivalent when processing is finished.^^J%
}
\fi

\typeout{Processing \wcFileName...^^J}

\IfFileExists{\wcFileName}{\batchmode}{\nonstopmode}
\edef\@tempa{\noexpand\makeatother
  \noexpand\input{\wcFileName}\noexpand\stop
}
\@tempa
"""

def is_first_line(line):
    if line.strip() == '':
        return False
    if '%' in line:
        return False
    return True

def count_main_text_words_detex(detex_lines, tex_lines):
    # remove images and empty lines
    detex_lines = [line for line in detex_lines if len(line.strip()) > 0]
    detex_lines = [line for line in detex_lines if '<Picture' not in line]

    title_line_no, = [i for i, line in enumerate(tex_lines) if '\maketitle' in line]
    first_line_no = title_line_no + 1
    while not is_first_line(tex_lines[first_line_no]):
        first_line_no += 1
    first_line = tex_lines[first_line_no]

    detex_first_line_no = 0
    for line in detex_lines:
        if line.strip() == first_line.strip():
            break
        detex_first_line_no += 1

    main_text = detex_lines[detex_first_line_no:]

    main_text = [line.replace('-', ' ') for line in main_text ] # hyphenated words count as two words
    lines_words = [line.split() for line in main_text]
    words = [word for words in lines_words for word in words ]

    #words_file = open('words', 'w')
    #words_file.writelines([word+'\n' for word in words])
    #words_file.close()

    main_text_words = len(words)
    return main_text_words

def count_main_text_words_wordcount(tex_lines, opts):
    """
    Count words in main text following method described at

    http://journals.aps.org/authors/length-guide-faq
    """
    mod_tex_lines = tex_lines[:]

    # Commenting out the \maketitle command
    mod_tex_lines = [ line.replace(r'\maketitle', r'%\maketitle') for line in mod_tex_lines ]

    # Using the 'nofootinbib' option
    mod_tex_lines = [ line.replace(r'\documentclass[', r'\documentclass[nofootbib, ')
                                    for line in mod_tex_lines ]
    # Putting an \end{document} before the bibliography
    bib_index = [ i for (i, line) in enumerate(mod_tex_lines) if r'\bibliography{' in line]
    if bib_index:
        mod_tex_lines.insert(bib_index[0], r'\end{document}' + '\n')

    # Putting an \end{document} before the acknowledgments/acknowledgements in environment \acknowledgments{...}
    ack_index = [ i for (i, line) in enumerate(mod_tex_lines) if r'\acknowle' in line]
    if ack_index:
        mod_tex_lines.insert(ack_index[0], r'\end{document}' + '\n')


    # Comment out any display equations and acknowledgments
    filterenvs = ['equation', 'eqnarray', 'align', 'displaymath', 'acknowledgments',
                  'acknowledgements', 'abstract', 'thebibliography']
    filtered_lines = []
    while mod_tex_lines:
        line = mod_tex_lines.pop(0)
        for env in filterenvs:
            if r'\begin{%s' % env in line:
                while mod_tex_lines and not r'\end{%s}' % env in line:
                    line = '% ' + line
                    filtered_lines.append(line)
                    line = mod_tex_lines.pop(0)
                line = '% ' + line
                filtered_lines.append(line)
                line = mod_tex_lines.pop(0) # comment out the \end too
        filtered_lines.append(line)

    mod_tex_lines = filtered_lines

    # FIXME - Commenting out the rows (but not the caption) of any tables

    tmp_tex_file = open('tmp_tex_file.tex', 'w')
    tmp_tex_file.writelines(line for line in mod_tex_lines)
    tmp_tex_file.close()

    wordcount_tex_file = open('wordcount.tex', 'w')
    wordcount_tex_file.write(wordcount_tex_contents)
    wordcount_tex_file.close()

    os.system('%s tmp_tex_file > /dev/null 2>&1' % opts.latex)
    os.system('bibtex tmp_tex_file > /dev/null 2>&1')
    os.system('%s tmp_tex_file > /dev/null 2>&1' % opts.latex)
    os.system('%s tmp_tex_file > /dev/null 2>&1' % opts.latex)
    os.system(r'echo tmp_tex_file.tex | %s wordcount.tex > /dev/null 2>&1' % opts.latex)
    wordcount_log = open('wordcount.log').readlines()

    rm_files = glob.glob('wordcount*') + glob.glob('tmp_tex_file*')
    for file in rm_files:
        os.unlink(file)

    wordcount = len([line for line in wordcount_log if '3.08633' in line or '3.08635' in line])
    return wordcount

def find_equation_lines(tex_lines):
    return [i for (i, line) in enumerate(tex_lines) if (r'\begin{equation' in line or
                                                        r'\begin{eqnarray' in line or
                                                        r'\begin{align' in line or
                                                        r'\begin{displaymath' in line)]
def count_equation_words(lines, start_line):
    count = 1
    array = False
    array_lines = 0
    two_column = '*' in lines[start_line]
    if two_column:
        eqn_words_per_line = 32
    else:
        eqn_words_per_line = 16

    for line in lines[start_line+1:]:
        if (r'\end{equation' in line or
            r'\end{eqnarray' in line or
            r'\end{align' in line or
            r'\end{displaymath' in line):
            break
        if r'\\' in line:
            if not array:
                count += 1
            else:
                array_lines += 1
        if r'\begin{array}' in line:
            array = True
            array_lines = 0
        if r'\end{array}' in line:
            array = False

    if array_lines != 0:
        count *= array_lines

    return count*eqn_words_per_line

def count_equations_words(tex_lines):
    eqn_line_nos = find_equation_lines(tex_lines)
    eqn_words = [count_equation_words(tex_lines, eqn_line_no) for eqn_line_no in eqn_line_nos]
    print 'Equations: %r' % eqn_words
    return sum(eqn_words)

def find_table_lines(tex_lines):
    return [i for (i, line) in enumerate(tex_lines) if r'\begin{tabl' in line]

def count_table_words(tex_lines, table_line):
    two_column = 'table*' in tex_lines[table_line]
    count = 1
    for line in tex_lines[table_line:]:
        if r'\end{table' in line:
            break
        if r'\\' in line:
            count += 1
    if two_column:
        print 'Two-column table with %d lines' % count
        return int(13.*count + 26.)
    else:
        print 'Single-column table with %d lines' % count
        return int(6.5*count + 13.)

def count_tables_words(tex_lines):
    table_lines = find_table_lines(tex_lines)
    table_words = [ count_table_words(tex_lines, table_line) for table_line in table_lines ]
    print 'Tables: %r' % table_words
    return sum(table_words)


def count_figures_words(detex_lines, tex_lines, opts):
    if opts.var is None:
        tex_vars = {}
    else:
        tex_vars = dict(opts.var)

    fig_lines = [line for line in detex_lines if '<Picture' in line ]
    fig_words = []
    #figs = {}

    for fig_i, fig_line in enumerate(fig_lines):
        filename = fig_line.strip()[1:-1].split()[1]
        this_fig_lines = [ (i, line) for i, line in enumerate(tex_lines) if filename in line and
                           ('input' in line or 'includegraphics' in line)]
        (inc_fig_line_no, inc_fig_line) = this_fig_lines[0]
        fig_line_no = inc_fig_line_no
        while r'\begin{figure' not in tex_lines[fig_line_no]:
            fig_line_no -= 1
        two_column = 'figure*' in tex_lines[fig_line_no]

        subfig = 'subfloat' in tex_lines[inc_fig_line_no]
        newline = r'\\' in tex_lines[inc_fig_line_no]

        #print filename, tex_lines[inc_fig_line_no], tex_lines[fig_line_no]

        for key in tex_vars.keys():
            if key in filename:
                filename = filename.replace(key, tex_vars[key])

        for ext in ['', '.pdf', '.eps', '.png']:
            if len(glob.glob(filename+ext)) == 1:
                break
        else:
            raise IOError('missing picture file %s' % filename)
        filename = filename+ext

        if opts.figs == 'identify':
            identify = subprocess.Popen(['identify', filename],
                                        stdout=subprocess.PIPE)
            out, err = identify.communicate()
            fields = out.split()
            width, height = fields[2].split('x')
            width = float(width)
            height = float(height)
        elif opts.figs == 'gs':
            img_f = open(filename, 'r')
            gs = subprocess.Popen(['gs', '-q', '-dSAFER', '-dBATCH', '-sDEVICE=bbox', '-'],
                                  stdin=img_f, stdout=subprocess.PIPE, stderr=subprocess.PIPE)
            out, err = gs.communicate()
            img_f.close()
            bbox = err.split('\n')[0].split()
            width = float(bbox[3])
            height = float(bbox[4])
        else:
            raise ValueError('Unknown figure method "%s"' % opts.figs)

        #if fig_line_no not in figs:
        #    figs[fig_line_no] = (fig_i, two_column, [(width, height, newline, filename)])
        #else:
        #    figs[fig_line_no][2].append((width, height, newline, filename))

        aspect = float(width/height)

        if two_column:
            words_equiv = 300./(0.5*aspect) + 40.
        else:
            words_equiv = 150./aspect + 20.

        print 'Figure %d:   %6d words (%.0fx%.0f aspect %.2f, %s)' % (fig_i+1, int(words_equiv),
                                                                      width, height,
                                                                      aspect, filename)
        fig_words.append(words_equiv)

    return int(sum(fig_words)*opts.scale_figs)


def count_chars_abstract(tex_lines):
    abs_begin_line, = [i for (i,line) in enumerate(tex_lines) if r'\begin{abstract}' in line]
    abs_end_line, = [i for (i,line) in enumerate(tex_lines) if r'\end{abstract}' in line]

    abstract_lines = tex_lines[abs_begin_line+1:abs_end_line]
    abstract_lines = [line for line in abstract_lines if not line.startswith('%') ]
    abstract = ''.join(abstract_lines)
    print 'ABSTRACT:'
    print abstract
    return len(abstract)


def process(tex_file, opts):
    print 'Processing TeX file: %s\n' % tex_file
    detex = subprocess.Popen(['detex', '-e', opts.env, tex_file],
                             stdout=subprocess.PIPE)
    out, err = detex.communicate()
    detex_lines = out.strip().split('\n')

    tex_lines = open(tex_file).readlines()

    abstract_chars = count_chars_abstract(tex_lines)
    print
    print 'Abstract:    %6d chars (max 600)' % abstract_chars
    print

    if opts.method == 'detex':
        main_text_words = count_main_text_words_detex(detex_lines, tex_lines)
    elif opts.method == 'wordcount':
        main_text_words = count_main_text_words_wordcount(tex_lines, opts)
    else:
        raise ValueError('Unsupported method %s' % opts.method)
    eqn_words = count_equations_words(tex_lines)
    fig_words = count_figures_words(detex_lines, tex_lines, opts)
    table_words = count_tables_words(tex_lines)
    total_words = (main_text_words + eqn_words + fig_words + table_words)

    print
    print 'Main text:      %6d words' % main_text_words
    print 'Displayed Math: %6d words' % eqn_words
    print 'Figures:        %6d words' % fig_words
    print 'Tables:         %6d words' % table_words
    print 'TOTAL:          %6d words' % total_words
    print
    wl = word_limit[opts.journal]
    if total_words > wl:
        over_under = 'OVER'
    else:
        over_under = 'UNDER'
    print ('Manuscript %s is currently %d words (%.0f%%) %s limit of %d words for journal %s' %
           (tex_file, abs(total_words - wl),
            float(total_words - wl)/wl*100., over_under,
            wl, opts.journal))


parser = optparse.OptionParser(usage='%prog [options] tex-files',
                               description="""
Count length of an APS manuscript formatted in LaTeX, following
guidelines described at http://journals.aps.org/authors/length-guide""")

parser.add_option('-v', '--var', metavar='key value', nargs=2, action='append',
                help='Define TeX variables e.g. to specify location of figure files.')
parser.add_option('-e', '--env', metavar='env1,env2,...',
                help='Comma-separated list of LaTeX environments to ignore.',
                default='abstract,acknowledgments,acknowledgements,displaymath,equation,eqnarray,thebibliography')
parser.add_option('-m', '--method', metavar='(detex | wordcount)', default='wordcount',
                  help='''Tool to use to count words in main text. Default is wordcount.
detex is also supported (but tends to underestimate word count).''')
parser.add_option('-f', '--figs', metavar='(identify | gs)',
                  help='''Tool to use to extract bounding box from figure.
The default is identify, which works for png, pdf, eps, and most image formats, but requires 
ImageMagick to be installed. The other option is gs, which works with eps and pdf mages.''',
                  default='identify')
parser.add_option('--scale-figs', type=float, default=1.1,
                  help='Scale estimate of figure word counts by factor, default 1.1 (10%)')
parser.add_option('-j', '--journal', metavar='PRL', default='PRL',
                  help='Journal abbreviation (e.g. PRL, PRB-RC)')
parser.add_option('-l', '--latex', default='pdflatex',
                  help='Latex executable. Default is "pdflatex".')


opts, args = parser.parse_args()

orig_eps_pdf_files = glob.glob('*-eps-converted-to.pdf')

for tex_file in args:
    process(tex_file, opts)

for eps_pdf_file in glob.glob('*-eps-converted-to.pdf'):
    if eps_pdf_file not in orig_eps_pdf_files:
        os.remove(delname)

